Categorical Semantics for Schr\"odinger's Equation

Applying ideas from monadic dynamics to the well-established framework of categorical quantum mechanics, we provide a novel toolbox for the simulation of finite-dimensional quantum dynamics. We use strongly complementary structures to give a graphical characterisation of quantum clocks, their action on systems and the relevant energy observables, and we proceed to formalise the connection between unitary dynamics and projection-valued spectra. We identify the Weyl canonical commutation relations in the axioms of strong complementarity, and conclude the existence of a dual pair of time/energy observables for finite-dimensional quantum clocks, with the relevant uncertainty principle given by mutual unbias of the corresponding orthonormal bases. We show that Schr\"odinger's equation can be abstractly formulated as characterising the Fourier transforms of certain Eilenberg-Moore morphisms from a quantum clock to a quantum dynamical system, and we use this to obtain a generalised version of the Feynman's clock construction. We tackle the issue of synchronism of clocks and systems, prove conservation of total energy and give conditions for the existence of an internal time observable for a quantum dynamical system. Finally, we identify our treatment as part of a more general theory of simulated symmetries of quantum systems (of which our clock actions are a special case) and their conservation laws (of which energy is a special case).

==> modules/pictures/ConcreteHistoriesEMProofHomsHists1.tex <==
\begin{tikzpicture}
	\path[use as bounding box] (-0.5,-1) rectangle (11,5);
		\node (in_0) at (0,0) {$\timeobj$};
		\node [morphism] (Psi_0) at (0,3) {$\Psi$};
		\node (out_0) at (0,4.5) {$\SpaceH$};
		\draw (in_0) to (Psi_0) to (out_0);	

\end{tikzpicture}


==> modules/pictures/FreeHistories1.tex <==
\begin{tikzpicture}
    \path[use as bounding box] (-1,-1) rectangle (5.5,3.5);

		\node [style] (I) at (0,0) {$\tensorUnit$};
		\node [style] (H1) at (2.5,0) {$\SpaceH$};

		\draw [style=->]  (I) -- node [below] {$\psi$} (H1);

\end{tikzpicture}

